Discrete Distribution Estimation under User-level Local Differential Privacy

We study discrete distribution estimation under user-level local differential privacy (LDP). In user-level $\varepsilon$-LDP, each user has $m\ge1$ samples and the privacy of all $m$ samples must be preserved simultaneously. We resolve the following dilemma: While on the one hand having more samples per user should provide more information about the underlying distribution, on the other hand, guaranteeing the privacy of all $m$ samples should make the estimation task more difficult. We obtain tight bounds for this problem under almost all parameter regimes. Perhaps surprisingly, we show that in suitable parameter regimes, having $m$ samples per user is equivalent to having $m$ times more users, each with only one sample. Our results demonstrate interesting phase transitions for $m$ and the privacy parameter $\varepsilon$ in the estimation risk. Finally, connecting with recent results on shuffled DP, we show that combined with random shuffling, our algorithm leads to optimal error guarantees (up to logarithmic factors) under the central model of user-level DP in certain parameter regimes. We provide several simulations to verify our theoretical findings.

==> related_work.tex <==
Turning to privacy at user-level, \cite{liu2020user} studies discrete distribution estimation under user-level central DP. They showed that under certain parameter regimes, the estimation risk scales as $\tilde{O}(\sqrt{\ab/ (\ns \nspu)} + \ab/(\ns \sqrt{\nspu}\eps))$, which also improves by $\sqrt{\nspu}$. Note that the second term has a different dependence on $\ns$ than the LDP setting.

\cite{ACLST:21} studies a similar problem under communication constraints where each user sends a message of at most $\ell$ bits. They show that more samples per user decreases the error by $O(1/\sqrt{\nspu})$ in certain parameter regimes. Our algorithm for $\eps \le 1$ is inspired by the algorithm in \cite{ACLST:21} with $\ell = 1$. A key difference is that we design a new localization scheme using sparse distribution estimation~\cite{pmlr-v132-acharya21b}, which is much simpler than one based on Gray code in \cite{ACLST:21}. Our lower bound uses the same hard instances as in \cite{ACLST:21}, while we need to deal with extra difficulties involved with LDP constraints. See \cref{sec:lower-bound} for a detailed discussion.
